MITP Colours in Darkness workshop summary report

This report summarises the talks and discussions that took place over the course of the MITP Youngst@rs Colours in Darkness workshop 2023. All talks can be found at https://indico.mitp.uni-mainz.de/event/377/.

==> Conclusions.tex <==
\section{Summary and Perspectives}

In this report, we have summarised the workshop....

